Red Supergiant Stars as Cosmic Abundance Probes: NLTE Effects in J-band Iron and Titanium Lines

Detailed non-LTE calculations for red supergiant stars are presented to investigate the influence of NLTE on the formation of atomic iron and titanium lines in the J-band. With their enormous brightness at J-band red supergiant stars are ideal probes of cosmic abundances. Recent LTE studies have found that metallicities accurate to 0.15 dex can be determined from medium resolution spectroscopy of individual red supergiants in galaxies as distant as 10 Mpc. The non-LTE results obtained in this investigation support these findings. Non-LTE abundance corrections for iron are smaller than 0.05 dex for effective temperatures between 3400K to 4200K and 0.1 dex at 4400K. For titanium the non-LTE abundance corrections vary smoothly between -0.4 dex and +0.2 dex as a function of effective temperature. For both elements, the corrections also depend on stellar gravity and metallicity. The physical reasons behind the non-LTE corrections and the consequences for extragalactic J-band abundance studies are discussed.

==> tab2.tex <==
%
% -----------NLTE ABUNDANCE CORRECTIONS v_turb=2 km/s-------------
%

\begin{deluxetable}{ccccccccc}
\tabletypesize{\scriptsize}
\tablecolumns{9}
\tablewidth{0pt}
\tablecaption{Non-LTE abundance corrections for the \tii\ and \fei\ lines ($\xi$ = 2 kms$^{-1}$)}

\tablehead{
\colhead{T$_{\rm eff}$}     &
\colhead{$log~g$}            &
\colhead{[Z]}           &
\colhead{$\Delta_{\rm Ti I}$}     &
\colhead{$\Delta_{\rm Ti I}$}             &
\colhead{$\Delta_{\rm Fe I}$}     &
\colhead{$\Delta_{\rm Fe I}$}             &
\colhead{$\Delta_{\rm Fe I}$}     &
\colhead{$\Delta_{\rm Fe I}$}\\
\colhead{}     &
\colhead{}            &
\colhead{}           &
\colhead{$11892.85$}     &
\colhead{$11949.58$}     &
\colhead{$11593.55$}             &
\colhead{$11638.25$}     &
\colhead{$11882.80$}             &
\colhead{$11973.01$}\\[1mm]
\colhead{(1)}	&
\colhead{(2)}	&
\colhead{(3)}	&
\colhead{(4)}	&
\colhead{(5)}	&
\colhead{(6)}	&
\colhead{(7)}   &
\colhead{(8)}	&
\colhead{(9)}}	
\startdata
\\[-1mm]
 4400. & -0.50 &  0.50 &  0.26  &  0.26 &  0.02 &  0.02 &  0.02 &  0.02 \\
 4400. & -0.50 &  0.00 &  0.22  &  0.22 &  0.05 &  0.04 &  0.03 &  0.03 \\
 4400. & -0.50 & -0.50 &  0.15  &  0.16 &  0.12 &  0.10 &  0.08 &  0.07 \\
 4400. &  0.00 &  0.50 &  0.19  &  0.18 &  0.01 &  0.01 &  0.01 &  0.01 \\
 4400. &  0.00 &  0.00 &  0.17  &  0.16 &  0.05 &  0.03 &  0.02 &  0.02 \\
 4400. &  0.00 & -0.50 &  0.12  &  0.12 &  0.11 &  0.09 &  0.07 &  0.06 \\
 4400. &  1.00 &  0.50 &  0.08  &  0.06 &  0.01 &  0.00 & -0.01 & -0.01 \\
 4400. &  1.00 &  0.00 &  0.09  &  0.08 &  0.03 &  0.02 &  0.01 &  0.01 \\
 4400. &  1.00 & -0.50 &  0.08  &  0.07 &  0.08 &  0.08 &  0.05 &  0.05 \\
 & & & & & & & & \\ 
%
 4200. & -0.50 &  0.50 &  0.17 &  0.15 &  0.00 &  0.00 &  0.01 &  0.01 \\
 4200. & -0.50 &  0.00 &  0.25 &  0.25 &  0.01 &  0.01 &  0.01 &  0.01 \\
 4200. & -0.50 & -0.50 &  0.23 &  0.24 &  0.04 &  0.03 &  0.02 &  0.02 \\
 4200. &  0.00 &  0.50 &  0.08 &  0.06 &  0.00 &  0.00 &  0.00 &  0.00 \\
 4200. &  0.00 &  0.00 &  0.17 &  0.16 &  0.01 &  0.00 &  0.00 &  0.01 \\
 4200. &  0.00 & -0.50 &  0.16 &  0.16 &  0.04 &  0.03 &  0.01 &  0.02 \\
 4200. &  1.00 &  0.50 &  0.04 & -0.07 &  0.00 & -0.01 & -0.01 & -0.01 \\
 4200. &  1.00 &  0.00 &  0.07 &  0.05 &  0.01 &  0.00 &  0.00 &  0.00 \\
 4200. &  1.00 & -0.50 &  0.09 &  0.08 &  0.03 &  0.02 &  0.01 &  0.01 \\
 & & & & & & & & \\
%
 4000. & -0.50 &  0.50 & -0.06 & -0.08 & -0.01 &  0.00 &  0.00 &  0.00 \\
 4000. & -0.50 &  0.00 &  0.12 &  0.10 &  0.00 & -0.01 &  0.00 &  0.00 \\
 4000. & -0.50 &  0.50 &  0.22 &  0.22 &  0.01 &  0.00 &  0.00 &  0.00 \\
 4000. &  0.00 &  0.50 & -0.13 & -0.15 & -0.01 & -0.01 & -0.01 &  0.00 \\
 4000. &  0.00 &  0.00 &  0.04 &  0.02 &  0.00 & -0.01 & -0.01 &  0.00 \\
 4000. &  0.00 & -0.50 &  0.15 &  0.14 &  0.01 &  0.00 &  0.00 &  0.00 \\
 4000. &  1.00 &  0.50 & -0.20 & -0.23 &  0.00 & -0.01 & -0.01 & -0.01 \\
 4000. &  1.00 &  0.00 & -0.05 & -0.08 &  0.00 & -0.01 & -0.01 & -0.01 \\
 4000. &  1.00 & -0.50 &  0.07 &  0.05 &  0.01 &  0.00 &  0.00 &  0.00 \\
 & & & & & & & & \\
%
 3800. & -0.50 &  0.50 & -0.24 & -0.26 & -0.01 & -0.01 & -0.01 &  0.00 \\
 3800. & -0.50 &  0.00 & -0.11 & -0.14 & -0.01 & -0.01 & -0.01 &  0.00 \\
 3800. & -0.50 & -0.50 &  0.08 &  0.06 &  0.00 & -0.01 & -0.01 & -0.01 \\
 3800. &  0.00 &  0.50 & -0.28 & -0.31 & -0.01 & -0.01 & -0.01 & -0.01 \\
 3800. &  0.00 &  0.00 & -0.17 & -0.20 & -0.01 & -0.01 & -0.01 & -0.01 \\
 3800. &  0.00 & -0.50 &  0.02 &  0.00 &  0.00 & -0.01 & -0.01 & -0.01 \\
 3800. &  1.00 &  0.50 & -0.31 & -0.33 &  0.00 & -0.01 & -0.02 & -0.01 \\
 3800. &  1.00 &  0.00 & -0.21 & -0.24 &  0.00 & -0.01 & -0.01 & -0.01 \\
 3800. &  1.00 & -0.50 & -0.04 & -0.07 &  0.00 &  0.00 & -0.01 & -0.01 \\
 & & & & & & & & \\
%
 3400. & -0.50 &  0.50 & -0.36 & -0.36 & -0.01 & -0.01 & -0.01 & -0.01 \\
 3400. & -0.50 &  0.00 & -0.38 & -0.40 & -0.01 & -0.02 & -0.01 & -0.01 \\
 3400. & -0.50 & -0.50 & -0.32 & -0.35 & -0.01 & -0.02 & -0.02 & -0.01 \\
 3400. &  0.00 &  0.50 & -0.36 & -0.37 & -0.01 & -0.01 & -0.01 & -0.01 \\
 3400. &  0.00 &  0.00 & -0.38 & -0.41 & -0.01 & -0.02 & -0.02 & -0.01 \\
 3400. &  0.00 & -0.50 & -0.32 & -0.35 & -0.01 & -0.02 & -0.02 & -0.01 \\
 3400. &  1.00 &  0.50 & -0.30 & -0.31 &  0.00 & -0.01 & -0.01 & -0.01 \\
 3400. &  1.00 &  0.00 & -0.29 & -0.32 &  0.00 & -0.01 & -0.01 & -0.01 \\
 3400. &  1.00 & -0.50 & -0.22 & -0.26 &  0.00 & -0.01 & -0.01 & -0.01 \\
%
\enddata
\end{deluxetable}


==> tab3.tex <==
%
% -----------NLTE ABUNDANCE CORRECTIONS v_turb=5 km/s-------------
%

\begin{deluxetable}{ccccccccc}
\tabletypesize{\scriptsize}
\tablecolumns{9}
\tablewidth{0pt}
\tablecaption{Non-LTE abundance corrections for the \tii\ and \fei\ lines ($\xi$ = 5 kms$^{-1}$)}

\tablehead{
\colhead{T$_{\rm eff}$}     &
\colhead{$log~g$}            &
\colhead{[Z]}           &
\colhead{$\Delta_{\rm Ti I}$}     &
\colhead{$\Delta_{\rm Ti I}$}             &
\colhead{$\Delta_{\rm Fe I}$}     &
\colhead{$\Delta_{\rm Fe I}$}             &
\colhead{$\Delta_{\rm Fe I}$}     &
\colhead{$\Delta_{\rm Fe I}$}\\
\colhead{}     &
\colhead{}            &
\colhead{}           &
\colhead{$11892.85$}     &
\colhead{$11949.58$}     &
\colhead{$11593.55$}             &
\colhead{$11638.25$}     &
\colhead{$11882.80$}             &
\colhead{$11973.01$}\\[1mm]
\colhead{(1)}	&
\colhead{(2)}	&
\colhead{(3)}	&
\colhead{(4)}	&
\colhead{(5)}	&
\colhead{(6)}	&
\colhead{(7)}   &
\colhead{(8)}	&
\colhead{(9)}}	
\startdata
\\[-1mm]
 4400. & -0.50 &  0.00 &  0.25 &  0.25 &  0.03 &  0.03 &  0.03 &  0.03 \\
 4400. & -0.50 &  0.00 &  0.22 &  0.22 &  0.06 &  0.06 &  0.04 &  0.04 \\
 4400. & -0.50 & -0.50 &  0.17 &  0.16 &  0.12 &  0.12 &  0.11 &  0.11 \\
 4400. &  0.00 &  0.50 &  0.20 &  0.20 &  0.02 &  0.01 &  0.00 &  0.01 \\
 4400. &  0.00 &  0.00 &  0.17 &  0.17 &  0.06 &  0.05 &  0.03 &  0.03 \\
 4400. &  0.00 & -0.50 &  0.15 &  0.14 &  0.11 &  0.11 &  0.10 &  0.10 \\
 4400. &  1.00 &  0.50 &  0.11 &  0.10 &  0.01 &  0.00 & -0.02 & -0.02 \\
 4400. &  1.00 &  0.00 &  0.11 &  0.11 &  0.04 &  0.03 &  0.02 &  0.01 \\
 4400. &  1.00 & -0.50 &  0.12 &  0.10 &  0.08 &  0.09 &  0.08 &  0.08 \\
 & & & & & & & & \\ 
%
 4200. & -0.50 &  0.50 &  0.19 &  0.18 &  0.00 &  0.00 &  0.00 &  0.00 \\
 4200. & -0.50 &  0.00 &  0.24 &  0.25 &  0.02 &  0.01 &  0.00 &  0.01 \\
 4200. & -0.50 & -0.50 &  0.22 &  0.23 &  0.05 &  0.04 &  0.02 &  0.03 \\
 4200. &  0.00 &  0.50 &  0.12 &  0.10 &  0.00 & -0.01 & -0.01 &  0.00 \\
 4200. &  0.00 &  0.00 &  0.18 &  0.18 &  0.02 &  0.01 & -0.01 &  0.00 \\
 4200. &  0.00 & -0.50 &  0.17 &  0.17 &  0.05 &  0.04 &  0.02 &  0.02 \\
 4200. &  1.00 &  0.50 &  0.02 & -0.01 &  0.00 & -0.01 & -0.02 & -0.02 \\
 4200. &  1.00 &  0.00 &  0.10 &  0.09 &  0.01 &  0.01 & -0.01 &  0.00 \\
 4200. &  1.00 & -0.50 &  0.11 &  0.11 &  0.03 &  0.03 &  0.02 &  0.02 \\
 & & & & & & & & \\
%
 4000. & -0.50 &  0.50 &  0.00 & -0.02 & -0.01 & -0.01 & -0.01 &  0.00 \\
 4000. & -0.50 &  0.00 &  0.15 &  0.14 &  0.00 & -0.01 & -0.02 &  0.00 \\
 4000. & -0.50 & -0.50 &  0.22 &  0.22 &  0.02 &  0.00 & -0.01 &  0.00 \\
 4000. &  0.00 &  0.50 & -0.06 & -0.09 & -0.01 & -0.01 & -0.02 & -0.01 \\
 4000. &  0.00 &  0.00 &  0.09 &  0.07 &  0.00 & -0.01 & -0.02 & -0.01 \\
 4000. &  0.00 & -0.50 &  0.16 &  0.16 &  0.02 &  0.01 & -0.01 &  0.00 \\
 4000. &  1.00 &  0.50 & -0.12 & -0.15 &  0.00 & -0.01 & -0.02 & -0.02 \\
 4000. &  1.00 &  0.00 &  0.01 & -0.01 &  0.00 &  0.00 & -0.01 & -0.01 \\
 4000. &  1.00 & -0.50 &  0.10 &  0.09 &  0.01 &  0.01 &  0.00 &  0.00 \\
 & & & & & & & & \\
%

 3800. & -0.50 &  0.50 & -0.18 & -0.21 & -0.02 & -0.02 & -0.01 & -0.01 \\
 3800. & -0.50 &  0.00 & -0.05 & -0.07 & -0.01 & -0.02 & -0.01 & -0.01 \\
 3800. & -0.50 & -0.50 &  0.12 &  0.11 &  0.00 & -0.01 & -0.02 & -0.02 \\
 3800. &  0.00 &  0.50 & -0.21 & -0.25 & -0.01 & -0.02 & -0.02 & -0.01 \\
 3800. &  0.00 &  0.00 & -0.09 & -0.12 &  0.00 & -0.02 & -0.02 & -0.02 \\
 3800. &  0.00 & -0.50 &  0.07 &  0.05 &  0.00 & -0.01 & -0.02 & -0.02 \\
 3800. &  1.00 &  0.50 & -0.23 & -0.26 &  0.00 & -0.01 & -0.02 & -0.02 \\
 3800. &  1.00 &  0.00 & -0.12 & -0.15 &  0.00 & -0.01 & -0.01 & -0.01 \\
 3800. &  1.00 & -0.50 &  0.02 &  0.00 &  0.00 &  0.00 & -0.01 & -0.01 \\
 & & & & & & & & \\
%
 3400. & -0.50 &  0.50 & -0.33 & -0.36 & -0.02 & -0.02 & -0.02 & -0.01 \\
 3400. & -0.50 &  0.00 & -0.32 & -0.36 & -0.01 & -0.02 & -0.03 & -0.02 \\
 3400. & -0.50 & -0.50 & -0.24 & -0.28 & -0.01 & -0.02 & -0.04 & -0.03 \\
 3400. &  0.00 &  0.50 & -0.33 & -0.36 & -0.01 & -0.02 & -0.02 & -0.01 \\
 3400. &  0.00 &  0.00 & -0.31 & -0.35 & -0.01 & -0.02 & -0.03 & -0.02 \\
 3400. &  0.00 & -0.50 & -0.22 & -0.26 &  0.00 & -0.02 & -0.03 & -0.02 \\
 3400. &  1.00 &  0.50 & -0.25 & -0.28 &  0.00 & -0.01 & -0.01 & -0.01 \\
 3400. &  1.00 &  0.00 & -0.20 & -0.24 &  0.00 & -0.01 & -0.01 & -0.01 \\
 3400. &  1.00 & -0.50 & -0.12 & -0.15 &  0.00 &  0.00 & -0.01 & -0.01 \\
%
\enddata
\end{deluxetable}


==> tab4.tex <==
%
% -----------EQUIVALENT WIDTHS v_turb=2 km/s-------------
%

\begin{deluxetable}{ccccccccccccccc}
\tabletypesize{\scriptsize}
\tablecolumns{15}
\tablewidth{0pt}
\tablecaption{Equivalent widths \tablenotemark{a}  of the \tii\ and \fei\ lines ($\xi$ = 2 kms$^{-1}$)}

\tablehead{
\colhead{T$_{\rm eff}$}     &
\colhead{$log~g$}            &
\colhead{[Z]}           &
\colhead{$W_{\lambda,\rm Ti I}$}     &
\colhead{$W_{\lambda,\rm Ti I}$}             &
\colhead{$W_{\lambda,\rm Ti I}$}     &
\colhead{$W_{\lambda,\rm Ti I}$}             &
\colhead{$W_{\lambda,\rm Fe I}$}     &
\colhead{$W_{\lambda,\rm Fe I}$}             &
\colhead{$W_{\lambda,\rm Fe I}$}     &
\colhead{$W_{\lambda,\rm Fe I}$}             &
\colhead{$W_{\lambda,\rm Fe I}$}     &
\colhead{$W_{\lambda,\rm Fe I}$}             &
\colhead{$W_{\lambda,\rm Fe I}$}     &
\colhead{$W_{\lambda,\rm Fe I}$}\\
\colhead{}     &
\colhead{}            &
\colhead{}           &
\colhead{$11892$}     &
\colhead{$11892$}     &
\colhead{$11949$}     &
\colhead{$11949$}     &
\colhead{$11593$}             &
\colhead{$11593$}             &
\colhead{$11638$}     &
\colhead{$11638$}     &
\colhead{$11882$}             &
\colhead{$11882$}             &
\colhead{$11882$}             &
\colhead{$11973$}\\[1mm]
\colhead{}     &
\colhead{}            &
\colhead{}           &
\colhead{$LTE$}     &
\colhead{$NLTE$}     &
\colhead{$LTE$}     &
\colhead{$NLTE$}     &
\colhead{$LTE$}             &
\colhead{$NLTE$}             &
\colhead{$LTE$}     &
\colhead{$NLTE$}     &
\colhead{$LTE$}             &
\colhead{$NLTE$}             &
\colhead{$LTE$}             &
\colhead{$NLTE$}\\[1mm]
\colhead{(1)}	&
\colhead{(2)}	&
\colhead{(3)}	&
\colhead{(4)}	&
\colhead{(5)}	&
\colhead{(6)}	&
\colhead{(7)}   &
\colhead{(8)}	&
\colhead{(9)}	&
\colhead{(10)}   &
\colhead{(11)}	&
\colhead{(12)}	&
\colhead{(13)}   &
\colhead{(14)}	&
\colhead{(15)}}	
\startdata
\\[-1mm]
4400. & -0.50 &  0.50 & 221.6 & 186.3 & 239.7 & 205.6 & 438.5 & 436.0 & 492.1 & 488.2 & 658.1 & 649.8 &  773.3 &  759.5 \\    
4400. & -0.50 &  0.00 & 155.8 & 123.2 & 176.2 & 143.3 & 386.5 & 380.7 & 425.9 & 420.4 & 530.0 & 522.5 &  597.4 &  586.5 \\
4400. & -0.50 & -0.50 &  80.1 &  61.4 &  98.6 &  77.8 & 336.4 & 324.9 & 370.2 & 358.9 & 443.0 & 431.8 &  483.4 &  470.6 \\
4400. &  0.00 &  0.50 & 218.6 & 194.5 & 236.1 & 213.6 & 428.4 & 426.6 & 482.0 & 480.2 & 647.6 & 643.7 &  762.2 &  754.5 \\
4400. &  0.00 &  0.00 & 149.4 & 126.2 & 168.7 & 146.1 & 373.7 & 368.4 & 413.3 & 408.8 & 518.2 & 512.6 &  585.8 &  577.6 \\
4400. &  0.00 & -0.50 &  78.0 &  64.0 &  95.3 &  80.6 & 324.6 & 313.7 & 358.2 & 348.0 & 433.0 & 422.8 &  475.1 &  463.1 \\
4400. &  1.00 &  0.50 & 209.8 & 200.2 & 226.3 & 218.8 & 403.6 & 402.5 & 457.6 & 458.9 & 624.7 & 631.0 &  738.4 &  744.7 \\
4400. &  1.00 &  0.00 & 142.1 & 130.1 & 159.8 & 149.5 & 349.3 & 345.3 & 390.7 & 387.9 & 505.1 & 503.0 &  579.3 &  576.3 \\
4400. &  1.00 & -0.50 &  74.9 &  66.4 &  90.6 &  83.1 & 299.4 & 290.9 & 334.7 & 326.2 & 419.4 & 410.7 &  469.6 &  459.7 \\
& & & & & & & & & & & & & & \\
%
4200. & -0.50 &  0.50 & 264.6 & 245.8 & 280.5 & 263.8 & 472.3 & 472.3 & 546.2 & 545.1 & 783.9 & 779.7 &  950.8 &  942.1 \\
4200. & -0.50 &  0.00 & 210.5 & 177.0 & 228.4 & 196.2 & 411.1 & 409.4 & 459.9 & 458.6 & 603.5 & 600.7 &  702.4 &  696.1 \\
4200. & -0.50 & -0.50 & 141.5 & 106.9 & 162.0 & 126.6 & 362.2 & 357.7 & 399.4 & 396.0 & 490.9 & 487.2 &  548.5 &  542.7 \\
4200. &  0.00 &  0.50 & 256.3 & 247.7 & 271.9 & 265.6 & 454.1 & 454.5 & 524.3 & 525.2 & 749.0 & 749.4 &  906.0 &  904.0 \\
4200. &  0.00 &  0.00 & 199.5 & 177.5 & 217.0 & 196.5 & 394.0 & 392.3 & 441.8 & 441.3 & 581.2 & 580.8 &  675.9 &  673.1 \\
4200. &  0.00 & -0.50 & 130.9 & 107.7 & 150.1 & 127.3 & 345.5 & 341.1 & 382.9 & 379.6 & 475.6 & 472.5 &  533.6 &  529.0 \\
4200. &  1.00 &  0.50 & 237.4 & 241.5 & 252.5 & 259.2 & 414.3 & 414.4 & 479.0 & 482.1 & 685.5 & 694.9 &  827.7 &  838.1 \\
4200. &  1.00 &  0.00 & 183.7 & 175.7 & 200.2 & 194.1 & 361.9 & 360.5 & 410.4 & 410.3 & 553.8 & 555.1 &  650.6 &  652.0 \\
4200. &  1.00 & -0.50 & 119.4 & 107.9 & 137.0 & 126.8 & 315.8 & 312.5 & 356.0 & 353.0 & 461.8 & 458.5 &  529.5 &  525.8 \\
& & & & & & & & & & & & & & \\
%
4000. & -0.50 &  0.50 & 289.7 & 295.0 & 304.5 & 311.9 & 497.9 & 499.8 & 591.8 & 593.3 & 897.6 & 898.2 & 1110.4 & 1108.8 \\
4000. & -0.50 &  0.00 & 246.2 & 232.7 & 262.1 & 250.6 & 427.1 & 427.5 & 487.8 & 489.2 & 676.2 & 677.6 &  808.6 &  807.3 \\
4000. & -0.50 & -0.50 & 192.6 & 162.3 & 210.6 & 181.5 & 376.6 & 375.4 & 419.8 & 420.0 & 538.5 & 539.3 &  618.2 &  617.1 \\
4000. &  0.00 &  0.50 & 276.8 & 288.6 & 291.5 & 305.6 & 465.8 & 467.7 & 549.7 & 552.8 & 822.0 & 826.7 & 1011.3 & 1014.7 \\
4000. &  0.00 &  0.00 & 232.7 & 228.0 & 248.5 & 245.9 & 403.2 & 403.3 & 459.8 & 461.7 & 633.5 & 636.9 &  754.9 &  756.6 \\
4000. &  0.00 & -0.50 & 178.9 & 159.6 & 196.5 & 178.6 & 356.5 & 355.1 & 399.0 & 399.0 & 514.8 & 515.8 &  591.7 &  591.7 \\
4000. &  1.00 &  0.50 & 250.9 & 269.5 & 265.1 & 286.8 & 415.4 & 416.3 & 490.0 & 494.3 & 729.0 & 741.1 &  892.9 &  906.5 \\
4000. &  1.00 &  0.00 & 210.2 & 215.5 & 225.2 & 233.2 & 364.3 & 364.0 & 420.1 & 421.4 & 592.0 & 595.6 &  709.7 &  714.3 \\
4000. &  1.00 & -0.50 & 160.8 & 152.8 & 177.0 & 171.0 & 323.0 & 321.8 & 368.4 & 367.8 & 497.1 & 497.0 &  582.9 &  582.7 \\
& & & & & & & & & & & & & & \\
%
3800. & -0.50 &  0.50 & 302.3 & 324.7 & 316.6 & 341.2 & 503.8 & 507.2 & 610.7 & 614.4 & 956.9 & 961.1 & 1194.6 & 1196.6 \\
3800. & -0.50 &  0.00 & 265.7 & 277.3 & 280.4 & 294.3 & 429.0 & 430.8 & 499.2 & 502.6 & 719.8 & 724.9 &  875.6 &  879.2 \\
3800. & -0.50 & -0.50 & 225.4 & 216.2 & 241.2 & 234.1 & 378.7 & 378.9 & 427.7 & 430.0 & 570.1 & 574.2 &  669.2 &  671.9 \\
3800. &  0.00 &  0.50 & 286.7 & 312.8 & 300.8 & 329.5 & 466.3 & 469.2 & 560.2 & 564.9 & 862.8 & 870.6 & 1069.8 & 1077.1 \\
3800. &  0.00 &  0.00 & 250.4 & 266.9 & 264.8 & 284.1 & 401.1 & 402.2 & 465.4 & 468.9 & 665.5 & 671.7 &  805.7 &  810.8 \\
3800. &  0.00 & -0.50 & 211.6 & 209.7 & 227.1 & 227.6 & 356.6 & 356.5 & 404.1 & 405.9 & 541.1 & 544.8 &  634.9 &  638.2 \\
3800. &  1.00 &  0.50 & 257.1 & 285.8 & 271.0 & 303.0 & 408.6 & 409.7 & 489.3 & 494.2 & 746.7 & 760.4 &  921.5 &  937.4 \\
3800. &  1.00 &  0.00 & 223.1 & 242.9 & 237.0 & 260.3 & 357.8 & 357.9 & 419.9 & 421.7 & 612.4 & 617.1 &  744.8 &  751.1 \\
3800. &  1.00 & -0.50 & 187.8 & 192.4 & 202.5 & 209.9 & 320.2 & 320.0 & 370.9 & 371.4 & 520.6 & 522.1 &  621.9 &  623.7 \\
& & & & & & & & & & & & & & \\
%
3400. & -0.50 &  0.50 & 321.5 & 356.9 & 336.1 & 373.7 & 484.5 & 488.4 & 595.4 & 600.8 & 943.1 & 951.8 & 1179.0 & 1186.3 \\
3400. & -0.50 &  0.00 & 286.6 & 323.5 & 300.5 & 339.9 & 405.4 & 407.8 & 480.3 & 485.4 & 710.7 & 719.8 &  872.0 &  879.7 \\
3400. & -0.50 & -0.50 & 255.1 & 286.2 & 268.9 & 302.8 & 355.1 & 356.3 & 410.0 & 414.1 & 571.1 & 578.6 &  683.9 &  690.9 \\
3400. &  0.00 &  0.50 & 306.2 & 342.5 & 320.5 & 359.2 & 441.3 & 443.8 & 533.9 & 539.0 & 823.3 & 832.3 & 1021.3 & 1030.5 \\
3400. &  0.00 &  0.00 & 271.2 & 307.6 & 284.9 & 324.3 & 375.8 & 377.2 & 442.2 & 446.4 & 643.8 & 651.7 &  784.1 &  791.4 \\
3400. &  0.00 & -0.50 & 239.6 & 269.6 & 253.2 & 286.5 & 331.9 & 332.5 & 383.5 & 386.5 & 533.7 & 539.7 &  637.6 &  643.7 \\
3400. &  1.00 &  0.50 & 276.5 & 307.2 & 290.7 & 324.4 & 387.7 & 388.4 & 464.5 & 467.5 & 699.9 & 707.4 &  860.0 &  871.7 \\
3400. &  1.00 &  0.00 & 243.1 & 270.8 & 256.8 & 288.0 & 337.6 & 338.0 & 399.6 & 401.5 & 584.3 & 588.7 &  710.4 &  715.7 \\
3400. &  1.00 & -0.50 & 212.3 & 232.3 & 225.8 & 249.5 & 300.3 & 300.4 & 353.3 & 354.2 & 507.2 & 509.8 &  611.1 &  614.3 \\
%
\enddata
\tablenotetext{a}{equivalent widths $\EW$ are given in \mA}
\end{deluxetable}


==> tab5.tex <==
%
% -----------EQUIVALENT WIDTHS v_turb=5 km/s-------------
%

\begin{deluxetable}{ccccccccccccccc}
\tabletypesize{\scriptsize}
\tablecolumns{15}
\tablewidth{0pt}
\tablecaption{Equivalent widths \tablenotemark{a}  of the \tii\ and \fei\ lines ($\xi$ = 5 kms$^{-1}$)}

\tablehead{
\colhead{T$_{\rm eff}$}     &
\colhead{$log~g$}            &
\colhead{[Z]}           &
\colhead{$W_{\lambda,\rm Ti I}$}     &
\colhead{$W_{\lambda,\rm Ti I}$}             &
\colhead{$W_{\lambda,\rm Ti I}$}     &
\colhead{$W_{\lambda,\rm Ti I}$}             &
\colhead{$W_{\lambda,\rm Fe I}$}     &
\colhead{$W_{\lambda,\rm Fe I}$}             &
\colhead{$W_{\lambda,\rm Fe I}$}     &
\colhead{$W_{\lambda,\rm Fe I}$}             &
\colhead{$W_{\lambda,\rm Fe I}$}     &
\colhead{$W_{\lambda,\rm Fe I}$}             &
\colhead{$W_{\lambda,\rm Fe I}$}     &
\colhead{$W_{\lambda,\rm Fe I}$}\\
\colhead{}     &
\colhead{}            &
\colhead{}           &
\colhead{$11892$}     &
\colhead{$11892$}     &
\colhead{$11949$}     &
\colhead{$11949$}     &
\colhead{$11593$}             &
\colhead{$11593$}             &
\colhead{$11638$}     &
\colhead{$11638$}     &
\colhead{$11882$}             &
\colhead{$11882$}             &
\colhead{$11882$}             &
\colhead{$11973$}\\[1mm]
\colhead{}     &
\colhead{}            &
\colhead{}           &
\colhead{$LTE$}     &
\colhead{$NLTE$}     &
\colhead{$LTE$}     &
\colhead{$NLTE$}     &
\colhead{$LTE$}             &
\colhead{$NLTE$}             &
\colhead{$LTE$}     &
\colhead{$NLTE$}     &
\colhead{$LTE$}             &
\colhead{$NLTE$}             &
\colhead{$LTE$}             &
\colhead{$NLTE$}\\[1mm]
\colhead{(1)}	&
\colhead{(2)}	&
\colhead{(3)}	&
\colhead{(4)}	&
\colhead{(5)}	&
\colhead{(6)}	&
\colhead{(7)}   &
\colhead{(8)}	&
\colhead{(9)}	&
\colhead{(10)}   &
\colhead{(11)}	&
\colhead{(12)}	&
\colhead{(13)}   &
\colhead{(14)}	&
\colhead{(15)}}	
\startdata
\\[-1mm]

4400. & -0.50 &  0.50 & 387.6 & 304.7 & 432.6 & 349.8 & 871.8 & 866.0 &  944.3 &  938.2 & 1111.8 & 1106.5 & 1208.6 & 1198.9 \\
4400. & -0.50 &  0.00 & 234.0 & 170.0 & 278.6 & 209.9 & 781.9 & 768.3 &  850.8 &  838.4 &  990.4 &  980.0 & 1060.6 & 1047.5 \\
4400. & -0.50 & -0.50 &  96.0 &  68.2 & 123.1 &  91.3 & 678.3 & 651.4 &  748.6 &  722.2 &  877.9 &  853.4 &  936.3 &  910.1 \\
4400. &  0.00 &  0.50 & 385.6 & 324.5 & 428.4 & 369.3 & 847.7 & 843.4 &  920.2 &  917.0 & 1088.4 & 1087.5 & 1186.2 & 1181.5 \\
4400. &  0.00 &  0.00 & 225.4 & 176.5 & 268.0 & 216.7 & 751.8 & 739.6 &  820.4 &  809.8 &  960.5 &  952.4 & 1031.2 & 1020.8 \\
4400. &  0.00 & -0.50 &  95.4 &  71.8 & 123.1 &  95.8 & 650.4 & 626.3 &  719.7 &  695.9 &  849.0 &  826.7 &  907.9 &  883.9 \\
4400. &  1.00 &  0.50 & 373.1 & 341.7 & 412.8 & 384.9 & 788.0 & 785.0 &  860.8 &  860.8 & 1032.7 & 1039.7 & 1131.8 & 1143.2 \\
4400. &  1.00 &  0.00 & 217.2 & 186.4 & 257.1 & 226.7 & 691.1 & 682.5 &  759.8 &  752.4 &  904.7 &  900.3 &  979.8 &  974.8 \\
4400. &  1.00 & -0.50 &  94.4 &  76.1 & 120.6 & 100.8 & 589.6 & 571.8 &  657.4 &  639.0 &  789.7 &  771.0 &  852.7 &  833.0 \\
& & & & & & & & & & & & & & \\
%
4200. & -0.50 &  0.50 & 501.9 & 447.7 & 540.4 & 490.4 & 909.4 & 909.5 &  990.8 &  990.8 & 1200.4 & 1201.7 & 1335.5 & 1332.5 \\
4200. & -0.50 &  0.00 & 365.1 & 285.2 & 409.4 & 330.0 & 822.3 & 818.1 &  893.6 &  891.0 & 1050.7 & 1050.9 & 1138.6 & 1135.6 \\
4200. & -0.50 & -0.50 & 203.1 & 139.8 & 246.5 & 176.5 & 733.2 & 722.6 &  802.8 &  794.1 &  937.3 &  931.5 & 1003.0 &  995.8 \\
4200. &  0.00 &  0.50 & 485.0 & 453.6 & 522.5 & 495.5 & 873.7 & 873.8 &  953.8 &  955.5 & 1157.9 & 1163.3 & 1286.9 & 1289.0 \\
4200. &  0.00 &  0.00 & 343.8 & 288.4 & 386.6 & 332.5 & 784.4 & 780.1 &  855.5 &  853.5 & 1011.3 & 1013.2 & 1097.7 & 1097.3 \\
4200. &  0.00 & -0.50 & 186.6 & 142.0 & 227.0 & 178.7 & 693.7 & 683.6 &  763.4 &  754.8 &  899.0 &  893.1 &  965.4 &  958.6 \\
4200. &  1.00 &  0.50 & 446.4 & 441.8 & 481.8 & 482.4 & 792.3 & 791.8 &  869.9 &  872.9 & 1065.3 & 1076.8 & 1186.0 & 1202.6 \\
4200. &  1.00 &  0.00 & 316.4 & 288.9 & 355.5 & 331.1 & 708.0 & 704.9 &  779.2 &  777.6 &  938.7 &  940.5 & 1028.2 & 1030.0 \\
4200. &  1.00 & -0.50 & 172.0 & 144.4 & 208.5 & 180.6 & 619.4 & 612.3 &  689.6 &  682.8 &  832.1 &  826.0 &  904.9 &  898.5 \\
& & & & & & & & & & & & & & \\
%
4000. & -0.50 &  0.50 & 569.2 & 568.3 & 603.6 & 607.9 & 923.5 & 926.7 & 1016.2 & 1019.7 & 1274.3 & 1280.9 & 1447.7 & 1450.3 \\
4000. & -0.50 &  0.00 & 462.2 & 419.8 & 500.4 & 462.2 & 836.8 & 836.8 &  913.1 &  915.3 & 1095.2 & 1101.4 & 1206.9 & 1210.0 \\
4000. & -0.50 & -0.50 & 325.4 & 253.6 & 369.5 & 297.7 & 757.3 & 754.0 &  827.8 &  826.9 &  973.3 &  976.3 & 1051.0 & 1052.3 \\
4000. &  0.00 &  0.50 & 541.0 & 553.5 & 574.7 & 592.9 & 873.5 & 875.9 &  960.3 &  965.1 & 1195.8 & 1206.0 & 1351.4 & 1359.1 \\
4000. &  0.00 &  0.00 & 433.4 & 410.5 & 470.6 & 452.2 & 790.2 & 789.6 &  864.6 &  866.9 & 1038.5 & 1045.8 & 1142.4 & 1148.2 \\
4000. &  0.00 & -0.50 & 299.0 & 249.9 & 340.8 & 293.2 & 712.0 & 708.7 &  782.3 &  780.9 &  927.0 &  929.1 & 1003.6 & 1004.9 \\
4000. &  1.00 &  0.50 & 484.8 & 509.6 & 517.1 & 548.6 & 776.5 & 776.9 &  858.9 &  863.4 & 1076.3 & 1090.8 & 1216.0 & 1236.6 \\
4000. &  1.00 &  0.00 & 387.5 & 385.1 & 422.3 & 425.1 & 700.9 & 700.0 &  774.9 &  775.6 &  949.6 &  954.4 & 1053.9 & 1059.4 \\
4000. &  1.00 & -0.50 & 266.9 & 240.2 & 305.2 & 281.2 & 627.3 & 625.0 &  699.0 &  697.2 &  851.9 &  851.5 &  935.5 &  935.1 \\
& & & & & & & & & & & & & & \\
%
3800. & -0.50 &  0.50 & 603.1 & 640.5 & 635.2 & 678.4 & 911.2 & 916.4 & 1010.8 & 1017.0 & 1297.9 & 1309.1 & 1496.8 & 1504.5 \\
3800. & -0.50 &  0.00 & 517.4 & 529.1 & 551.4 & 568.9 & 825.1 & 827.3 &  905.7 &  910.8 & 1107.1 & 1117.9 & 1236.3 & 1244.2 \\
3800. & -0.50 & -0.50 & 416.5 & 383.6 & 454.6 & 425.8 & 753.5 & 753.3 &  825.3 &  828.1 &  981.9 &  989.7 & 1071.6 & 1077.8 \\
3800. &  0.00 &  0.50 & 568.4 & 612.0 & 600.0 & 650.2 & 854.0 & 857.6 &  946.4 &  953.2 & 1204.7 & 1218.7 & 1379.3 & 1390.9 \\
3800. &  0.00 &  0.00 & 483.8 & 505.1 & 517.0 & 544.7 & 772.4 & 773.4 &  850.1 &  854.5 & 1039.7 & 1050.5 & 1159.0 & 1168.1 \\
3800. &  0.00 & -0.50 & 387.6 & 370.2 & 424.3 & 411.6 & 705.1 & 704.5 &  776.4 &  778.1 &  930.5 &  936.6 & 1017.6 & 1023.3 \\
3800. &  1.00 &  0.50 & 503.2 & 548.5 & 533.8 & 586.9 & 749.0 & 750.1 &  835.1 &  840.2 & 1069.5 & 1085.2 & 1223.1 & 1245.8 \\
3800. &  1.00 &  0.00 & 425.1 & 451.0 & 456.7 & 489.7 & 675.2 & 675.2 &  751.9 &  753.7 &  941.0 &  947.2 & 1059.1 & 1066.0 \\
3800. &  1.00 & -0.50 & 340.0 & 335.1 & 373.9 & 374.4 & 613.1 & 612.4 &  685.8 &  685.9 &  849.5 &  851.4 &  944.5 &  946.8 \\
& & & & & & & & & & & & & & \\
%
3400. & -0.50 &  0.50 & 649.2 & 716.7 & 680.0 & 753.4 & 859.6 & 864.9 &  965.0 &  972.8 & 1267.7 & 1282.9 & 1476.4 & 1488.3 \\
3400. & -0.50 &  0.00 & 573.1 & 641.5 & 603.9 & 679.1 & 764.9 & 767.9 &  849.6 &  856.7 & 1062.7 & 1077.2 & 1203.3 & 1215.3 \\
3400. & -0.50 & -0.50 & 501.6 & 554.8 & 533.1 & 593.5 & 693.4 & 694.8 &  767.9 &  773.1 &  936.1 &  948.2 & 1038.4 & 1049.4 \\
3400. &  0.00 &  0.50 & 615.3 & 682.6 & 645.9 & 719.8 & 802.6 & 805.7 &  897.3 &  904.3 & 1156.7 & 1171.4 & 1332.8 & 1345.8 \\
3400. &  0.00 &  0.00 & 538.5 & 603.5 & 569.1 & 641.6 & 714.4 & 715.9 &  794.6 &  800.0 &  989.7 & 1002.0 & 1114.8 & 1126.2 \\
3400. &  0.00 & -0.50 & 466.9 & 515.4 & 497.9 & 554.2 & 645.3 & 645.9 &  718.2 &  721.5 &  880.8 &  889.8 &  977.8 &  987.0 \\
3400. &  1.00 &  0.50 & 547.5 & 599.2 & 578.1 & 636.9 & 712.5 & 713.2 &  800.2 &  803.6 & 1027.0 & 1036.4 & 1174.8 & 1186.1 \\
3400. &  1.00 &  0.00 & 473.7 & 516.6 & 504.1 & 554.7 & 632.6 & 632.9 &  711.7 &  713.5 &  901.0 &  906.9 & 1019.3 & 1026.0 \\
3400. &  1.00 & -0.50 & 404.1 & 429.5 & 434.8 & 467.4 & 566.6 & 566.6 &  640.7 &  641.6 &  808.8 &  812.0 &  909.5 &  913.5 \\
%
\enddata
\tablenotetext{a}{equivalent widths $\EW$ are given in \mA}
\end{deluxetable}

